Competitive Algorithms for Block-Aware Caching

We study the block-aware caching problem, a generalization of classic caching in which fetching (or evicting) pages from the same block incurs the same cost as fetching (or evicting) just one page from the block. Given a cache of size $k$, and a sequence of requests from $n$ pages partitioned into given blocks of size $\beta\leq k$, the goal is to minimize the total cost of fetching to (or evicting from) cache. We show the following results: $\bullet$ For the eviction cost model, we show an $O(\log k)$-approximate offline algorithm, a $k$-competitive deterministic online algorithm, and an $O(\log^2 k)$-competitive randomized online algorithm. $\bullet$ For the fetching cost model, we show an integrality gap of $\Omega(\beta)$ for the natural LP relaxation of the problem, and an $\Omega(\beta + \log k)$ lower bound for randomized online algorithms. The strategy of ignoring the block-structure and running a classical paging algorithm trivially achieves an $O(\beta)$ approximation and an $O(\beta \log k)$ competitive ratio respectively for the offline and online-randomized setting. $\bullet$ For both fetching and eviction models, we show improved bounds for the $(h,k)$-bicriteria version of the problem. In particular, when $k=2h$, we match the performance of classical caching algorithms up to constant factors. Our results establish a separation between the tractability of the fetching and eviction cost models, which is interesting since fetching/evictions costs are the same up to an additive term for classic caching. Previous work only studied online deterministic algorithms for the fetching cost model when $k > h$. Our insight is to relax the block-aware caching problem to a submodular covering LP. The main technical challenge is to maintain a competitive fractional solution, and to round it with bounded loss, as the constraints of this LP are revealed online.

==> conclusion.tex <==
	\section{Conclusion and Open Questions}

\label{sec:conclusion}

In this work we significantly expand on known results of \cite{beckmann2021brief} for the block-aware caching problem. For the eviction cost model, we give the first set of algorithms avoiding a trivial multiplicative $\beta$ overhead over their classical paging counterparts. We also give $(h,k)$-bicriteria algorithms for both fetching and eviction cost models, which we in turn use to adapt the lower bound of \cite{beckmann2021brief} for the fetching cost model to randomized algorithms.

We leave the following as interesting open questions.

\begin{question}
Can our $O(\log^2 k)$ competitive ratio for block-caching in the eviction cost model be improved to $O(\log k)$ to match the lower bound from classical paging? 
\end{question}

Note that even for the special case of generalized caching, the first result of \cite{BBN08} achieved competitive ratio $O(\log^2 k)$. The subsequent improvement due to \cite{ACER19} required non-trivial ideas which seem difficult to adapt to the more general block-aware caching problem.

\begin{question}
Is there an algorithm for block-caching in the fetching cost model matching the lower bound of $\bsize+\log k$, or can the lower bound be strengthened to match the trivial $\bsize \log k$ upper bound?
\end{question}

\begin{question}
	Are there constant-approximation  \emph{offline} algorithms for block-caching in either the fetching or eviction cost models? 
\end{question}
